Design of High-Order Decoupled Multirate GARK Schemes

Multirate time integration methods apply different step sizes to resolve different components of the system based on the local activity levels. This local selection of step sizes allows increased computational efficiency while achieving the desired solution accuracy. While the multirate idea is elegant and has been around for decades, multirate methods are not yet widely used in applications. This is due, in part, to the difficulties raised by the construction of high order multirate schemes. Seeking to overcome these challenges, this work focuses on the design of practical high-order multirate methods using the theoretical framework of generalized additive Runge-Kutta (MrGARK) methods, which provides the generic order conditions and the linear and nonlinear stability analyses. A set of design criteria for practical multirate methods is defined herein: method coefficients should be generic in the step size ratio, but should not depend strongly on this ratio; unnecessary coupling between the fast and the slow components should be avoided; and the step size controllers should adjust both the micro- and the macro-steps. Using these criteria, we develop MrGARK schemes of up to order four that are explicit-explicit (both the fast and slow component are treated explicitly), implicit-explicit (implicit in the fast component and explicit in the slow one), and explicit-implicit (explicit in the fast component and implicit in the slow one). Numerical experiments illustrate the performance of these new schemes.

==> Include/GARK_simplifying_assumptions.tex <==

%%%%%%%%%%%%%%%%%%%%%%
\subsection{GARK simplifying assumptions}
%%%%%%%%%%%%%%%%%%%%%%

GARK simplifying assumptions seek to reduce the number of multicolored trees. They allow to express the coupling matrices as functions of the base coefficients such that many of the coupling conditions are eliminated.

%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Simplifying assumptions of type $C(k)$}
%%%%%%%%%%%%%%%%%%%%%%

We introduce the following GARK simplifying assumption:
%
\begin{eqnarray}
\label{eqn:simplifying-condition-C}
C(\ell,k): \qquad \mathbf{A}^{\{\sigma,\mu_1\}} \cdot \dots \cdot \mathbf{A}^{\{\mu_{\ell-1},\mu_\ell\}} \cdot \mathbf{c}^{\{\mu_\ell\} \times k}  &=&  \left( \mathbf{A}^{\{\sigma,\sigma\}} \right)^\ell \cdot \mathbf{c}^{\{\sigma\} \times k}, \quad \\
\nonumber
&&\quad \forall~ \sigma,\mu_1,\dots,\mu_\ell.
\end{eqnarray}
%

\begin{table}
\centering
\begin{tabular}{||c c c||}
    \hline\hline
    \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$$](j){$\sigma$}; [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\mathbf{A}^{\{\sigma,\nu\}}$](k){$\nu$}; [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\mathbf{c}^{\{\nu\}}$](m){$\nu$};  ][.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\mathbf{c}^{\{\nu\}}$](l){$\nu$};  ] ] ]\end{tikzpicture} & 
    $\longrightarrow$ &
    \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$$](j){$\sigma$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\mathbf{A}^{\{\sigma,\sigma\}}$](k){$\sigma$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\mathbf{c}^{\{\sigma\}}$](m){$\sigma$};  ][.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\mathbf{c}^{\{\sigma\}}$](l){$\sigma$};  ] ] ]\end{tikzpicture}\\ 
\hline\hline
%
        \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$$](j){$\sigma$}; [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\mathbf{A}^{\{\sigma,\mu_1\}}$](k){$\mu_1$}; [.\node[circle,draw,thick,fill=green!50,opacity=0.5,label=right:$\mathbf{A}^{\{\mu_1,\mu_2\}}$](l){$\mu_2$}; [.\node[circle,draw,thick,fill=green!50,opacity=0.5,label=right:$\mathbf{c}^{\{\mu_2\}}$](m){$\mu_2$};  ] ] ] ]\end{tikzpicture} &
            $\longrightarrow$ & 
         \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$$](j){$\sigma$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\mathbf{A}^{\{\sigma,\sigma\}}$](k){$\sigma$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\mathbf{A}^{\{\sigma,\sigma\}}$](l){$\sigma$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\mathbf{c}^{\{\sigma\}}$](m){$\sigma$};  ] ] ] ]\end{tikzpicture} \\ \hline\hline
%
\end{tabular}
\caption{How condition $C(\ell,k)$ \eqref{eqn:simplifying-condition-C} simplifies trees. In the upper two panels $\ell=1$ and $k=2$. In the lower two panels $\ell=2$ and $k=1$. The equation $\mathbf{A}^{\{\sigma,\mu\}} \cdot \mathbf{c}^{\{\mu\} \times k}  =  \mathbf{A}^{\{\sigma,\sigma\}} \cdot \mathbf{c}^{\{\sigma\} \times k}$ means that a subtree with $\ell+1$ levels, consisting of a linear branch that ends with $k$ leaves, gets the color of its root.}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Simplifying assumptions of type $D(k)$}
%%%%%%%%%%%%%%%%%%%%%%
%
\begin{eqnarray}
\label{eqn:simplifying-condition-D}
D(\ell,k): ~~ \left(\mathbf{b}^{\{\sigma\}} \times \mathbf{c}^{\{\sigma\} \times k}\right)^T  \cdot \mathbf{A}^{\{\sigma,\mu_1\}}\cdot \dots  \cdot \mathbf{A}^{\{\mu_{\ell-1},\mu_\ell\}} &=& \left(\mathbf{b}^{\{\mu_\ell\}} \times \mathbf{c}^{\{\mu_\ell\} \times k}\right)^T  \cdot \left( \mathbf{A}^{\{\mu_\ell,\mu_\ell\}} \right)^\ell, \quad \\
\nonumber
&& \qquad\forall~ \sigma,\mu_1,\dots,\mu_\ell.
\end{eqnarray}
%
The way condition $D(\ell,k)$ simplifies trees is illustrated in Table \ref{tab:simplifying-condition-D}.
%
\begin{table}[hp]
\centering
\begin{tabular}{||c c c ||}
    \hline\hline
    \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\mathbf{b}^{\{\sigma\}}\,^T$](j){$\sigma$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\mathbf{A}^{\{\sigma,\nu\}}$](l){$\sigma$};  ][.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\mathbf{c}^{\{\sigma\}}$](k){$\sigma$};  ] ]\end{tikzpicture} 
    & $\longrightarrow$ & 
    \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\mathbf{b}^{\{\nu\}}\,^T$](j){$\nu$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\mathbf{A}^{\{\nu,\nu\}}$](l){$\nu$};  ][.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\mathbf{c}^{\{\nu\}}$](k){$\nu$};  ] ]\end{tikzpicture} \\ 
    \hline\hline
\end{tabular}
\caption{How condition $D(\ell,k)$ simplifies trees. Here $\ell=k=1$. A tree has a root with $k+1$ children, out of which $k$ are leaves. The $k+1$-st is a subtree that starts with $\ell$ nodes in a linear pattern. The root takes the color of the $\ell$-th child of its $k+1$-st child.}
\label{tab:simplifying-condition-D}
\end{table}
%

\begin{comment}
For internally consistent MR-GARK methods satisfying the simplifying conditions \eqref{eqn:simplifying-condition-C-MR} with $k=1$:
%
\begin{itemize}
\item There are no coupling conditions of order 2.
\item There are no coupling conditions of order 3. This property is enjoyed equally by the main and by any embedded methods.
\item the order 4 conditions simplify considerably, as follows:
\begin{itemize}
\item The two trees in table \ref{tab:N2t41_intconsist} remain the same
\item Only $t_{4,2}^{\langle 2,1 \rangle}$ and $t_{4,2}^{\langle 2,16 \rangle}$ remain from the trees of table \ref{tab:N2t42_intconsist}
\item The four trees in table \ref{tab:N2t43_intconsist} remain the same
\item Only $t_{4,4}^{\langle 2,1 \rangle}$, $t_{4,4}^{\langle 2,8 \rangle}$, $t_{4,4}^{\langle 2,9 \rangle}$, $t_{4,4}^{\langle 2,16 \rangle}$ remain from the trees of table \ref{tab:N2t44_intconsist}.
\end{itemize}
\item Among the 11 trees for order 4 only $t_{4,3}^{\langle 2,6 \rangle}$, $t_{4,3}^{\langle 2,7 \rangle}$, $t_{4,4}^{\langle 2,8 \rangle}$, and $t_{4,4}^{\langle 2,9 \rangle}$ represent coupling conditions.
\end{itemize}
\end{comment}

\begin{comment}
For internally consistent MR-GARK methods satisfying the simplifying conditions \eqref{eqn:simplifying-condition-D-MR} with $k=0$:
%
\begin{itemize}
\item There are no coupling conditions of order 2.
\item There are no coupling conditions of order 3. This property is enjoyed equally by the main and by any embedded methods.
\item the order 4 conditions simplify considerably, as follows:
\begin{itemize}
\item The two trees in table \ref{tab:N2t41_intconsist} remain the same
\item Only $t_{4,2}^{\langle 2,1 \rangle}$ and $t_{4,2}^{\langle 2,16 \rangle}$ remain from the trees of table \ref{tab:N2t42_intconsist}
\item The four trees in table \ref{tab:N2t43_intconsist} remain the same
\item Only $t_{4,4}^{\langle 2,1 \rangle}$, $t_{4,4}^{\langle 2,8 \rangle}$, $t_{4,4}^{\langle 2,9 \rangle}$, $t_{4,4}^{\langle 2,16 \rangle}$ remain from the trees of table \ref{tab:N2t44_intconsist}.
\end{itemize}
\item Among the 11 trees for order 4 only $t_{4,3}^{\langle 2,6 \rangle}$, $t_{4,3}^{\langle 2,7 \rangle}$, $t_{4,4}^{\langle 2,8 \rangle}$, and $t_{4,4}^{\langle 2,9 \rangle}$ represent coupling conditions.
\end{itemize}
\end{comment}

\begin{comment}
For MR-GARK methods satisfying the simplifying conditions $C(1,0) \&C(1,1)\&D(1,0)$, or $C(1,0) \&C(1,1)\&C(2,1)$:
%
\begin{itemize}
\item There are no coupling conditions of order 2.
\item There are no coupling conditions of order 3. 
\item There are no coupling conditions of order 4.
\end{itemize}
\end{comment}



==> Include/MGARK_S_methods.tex <==

{\color{blue}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Methods of type S}
\label{sec:s_schemes}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%S stands for simplicity-stability. Criteria:
%\begin{itemize}
%\item Limit the increase of coupling coefficients when $M \to \infty$. Ideally they should remain bounded for all $M$.
%This helps stability.
%\item Maximize the sparsity of the coupling coefficients. This helps simplicity. It also helps the implementation and decreases data dependencies.
%\end{itemize}

%%%%%%%%%%%%%%EXEX21%%%%%%%%%%%%%%
\subsection{\mgark \method{\explicit}{\explicit}{2}{1}{2}{2}[S]}
\label{subsec:method_EXEX2s}
%%%%%%%%%%%%%%EXEX21%%%%%%%%%%%%%%
  This explicit method uses a base method from \cite{ralston1962runge} and has telescopic \cref{eqn:mr-telescopic-conditions} and naturally adaptive (\cref{def:naturally-adaptive}) properties.
  
The scheme computes the first slow stage, followed by $L$ fast steps, then the second slow stage, followed by $M-L_2$ fast steps.  For example $L_2 = floor(c_2  \, M)$.
  
\[
	\c^{\{\f\}} = \frac{1}{M} \left[ c^{\{\f\}} + \left(\lambda-1\right) \one  \right]_{\lambda=1,\dots,M}.
\]  
  
\[
  	A^{\{\f,\f\}}=A^{\{\s,\s\}} =
	  	\begin{bmatrix}
	  	0 & 0 \\
	  	c_2 & 0 \\
	  	\end{bmatrix}, \quad
		 	b^{{\{\f\}}} =   b^{{\{\s\}}} =
	  	\begin{bmatrix}
	  	 \frac{2\,c_2-1}{2\,c_2} & \frac{1}{2\,c_2} \\
	  	\end{bmatrix}\trsym,
		\quad
    \widehat{b}^{{\{\f\}}}  =   \widehat{b}^{{\{\s\}}} =
	    \begin{bmatrix}
	    1 & 0 \\
	    \end{bmatrix}\trsym.
\]
%
\[
  A^{\{\f,\s,\lambda\}}  = 
  \begin{cases}
  \frac{1}{M}\,
	  	\begin{bmatrix}
	  	\left(\lambda-1\right) & 0 \\
	  	c_2 + \left(\lambda-1\right) & 0 
	  	\end{bmatrix}, & 1 \le \lambda \le L_2, \\[12pt]
\frac{1}{M}\,
	  	\begin{bmatrix}
	  	0 & \left(\lambda-1\right)  \\
	  	0 & c_2 + \left(\lambda-1\right)  
	  	\end{bmatrix}, & L_2+1 \le \lambda \le M.
\end{cases}		
\]
%	  	\end{bmatrix},$
\[
  A^{\{\s,\f,\lambda\}}  = 
  \begin{cases}
  \frac{1}{M}\,
	  	\begin{bmatrix}
	  	0 & 0 \\
	  	0 & 0 
	  	\end{bmatrix}, &  \lambda \ne L_2, \\[12pt]
\frac{1}{M}\,
	  	\begin{bmatrix}
	  	0 & 0  \\
	  	c_2 & 0
	  	\end{bmatrix}, & \lambda =L_2.
\end{cases}		
\]

\fitbox{2}{
	$A^{\{\f,\f\}}=
	\begin{bmatrix}
	0 & 0 \\
	c_2 & 0 \\
	\end{bmatrix},$
	&
	$A^{\{\s,\s\}} =
	\begin{bmatrix}
	0 & 0 \\
	c_2 & 0 \\
	\end{bmatrix},$
	\\
	$A^{\{\f,\s,\lambda\}} =
		\begin{bmatrix}
		\frac{\lambda -1}{M} & 0 \\
		\frac{\lambda +c_2-1}{M} & 0 \\
		\end{bmatrix},$
	& $\lambda = 1, \ldots, L_2, $  \\
	$A^{\{\f,\s,\lambda\}} =
	\begin{bmatrix}
	\frac{(\lambda -1) \left(2 c_2-1\right)}{2 M c_2} & \frac{\lambda -1}{2 M c_2} \\
	\frac{M}{3 \left(L_2-M\right)}+\frac{-\lambda +2 c_2 \left(2 \lambda +c_2-2\right)+1}{2 M c_2} & \frac{M}{3 M-3 L_2}+\frac{\lambda -1}{2 M c_2}+\frac{1-\lambda }{M} \\
	\end{bmatrix},$
	& $\lambda = L_2 + 1, \ldots, M, $  \\
	%%%%%%%%%%%%%%%%%%
	$A^{\{\s,\f,\lambda\}} =
	\begin{bmatrix}
	0 & 0 \\
	\frac{M \left(-2 M+6 c_2+3 L_2-3\right)}{6 L_2} & \frac{M \left(2 M-3 L_2+3\right)}{6 L_2} \\
	\end{bmatrix},$
	&
	$\lambda = 1, \ldots, L_2,$  \\
	%%%%%%%%%%%%%%%%%%
	$A^{\{\s,\f,\lambda\}} =
	\begin{bmatrix}
	0 & 0 \\
	0 & 0 \\
	\end{bmatrix},$
	&
	$\lambda = L_2 + 1, \ldots, M,$  \\
	%%%%%%%%%%%%%%%%%%
	$b^{{\{\f\}}} =   b^{{\{\s\}}} =
	\begin{bmatrix}
	\frac{2 c_2-1}{2 c_2} & \frac{1}{2 c_2} \\
	\end{bmatrix}\trsym,$
	&
	$\widehat{b}^{{\{\f\}}}  =   \widehat{b}^{{\{\s\}}} =
	\begin{bmatrix}
	1 & 0 \\
	\end{bmatrix}\trsym.$
}

\begin{figure}[ht!]
	\centering
	\begin{subfigure}[b]{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/Stability/ex2-ex2-2(1)S/m2-3d.pdf}
		\caption{$M=2$.}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.45\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/Stability/ex2-ex2-2(1)S/m4-3d.pdf}
		\caption{$M=4$.}
	\end{subfigure}
	\caption{\method{\explicit}{\explicit}{2}{1}{2}{2}[S] stability regions with $c_2 = \frac{2}{3}$.}
\end{figure}

%%%%%%%%%%%%%%EXEX21%%%%%%%%%%%%%%
\newpage
\subsection{\mgark \method{\explicit}{\explicit}{3}{2}{3}{3}[S]}
\label{subsec:method_EXEX3s}
%%%%%%%%%%%%%%EXEX21%%%%%%%%%%%%%%
This explicit method uses a base method from \cite{ralston1962runge} and has telescopic \cref{eqn:mr-telescopic-conditions} and naturally adaptive (\cref{def:naturally-adaptive}) properties.
  
The base method is 3 stages, order 3, with an embedded method of order 2:
%
%\[
%\quad
%\A = \begin{bmatrix}
% \frac{6 c_2 c_3-3 c_2-3 c_3+2}{6 c_2 c_3} \\
% \frac{2-3 c_3}{6 c_2^2-6 c_2 c_3} \\
% -\frac{2-3 c_2}{6 c_2 c_3-6 c_3^2}
%\end{bmatrix}
%\quad
%\begin{bmatrix}
% 0 \\
% c_2 \\
% c_3 
%\end{bmatrix}
% \] 
% 
% \[
%b= \begin{bmatrix}
% \frac{6 c_2 c_3-3 c_2-3 c_3+2}{6 c_2 c_3} \\
% \frac{2-3 c_3}{6 c_2^2-6 c_2 c_3} \\
% -\frac{2-3 c_2}{6 c_2 c_3-6 c_3^2} 
%\end{bmatrix}
%\quad
%\hat{b} = 
%\begin{bmatrix}
% \hat{b}_2 \left(\frac{c_2}{c_3}-1\right)-\frac{1}{2 c_3}+1 \\
% \hat{b}_2 \\
% \frac{1-2 \hat{b}_2 c_2}{2 c_3}
%\end{bmatrix}
% \]
  
Choose $L_2 = floor(c_2  \, M)$ and $L_3 = floor(c_3  \, M)$. The evaluation order is:
%
\begin{enumerate}
\item slow-stage-1,\item fast-steps-$1:L_2$,\item  slow-stage-2,\item  fast-steps-$L_2+1:L_3$, \item  slow-stage-3,
\item  fast-steps-$L_3+1:M$.
\end{enumerate}



\paragraph{Coupling order conditions}
	\begin{align*}
	\c^{\{\f\}} &= \frac{1}{M} \left[ c^{\{\f\}} + \left(\lambda-1\right) \one  \right]_{\lambda=1,\dots,M} \\
	%
	 \frac{M^{\phantom{.}}}{6} &= \sum_{\lambda=1}^M \tr{b^{\{\f\}}} \mprod A^{\{\f,\s,\lambda\}} \mprod c^{\{\s\}} \\
	%
	\frac{M^2}{6} &= \sum_{\lambda=1}^M \tr{b^{\{\s\}}} A^{\{\s,\f,\lambda\}} \mprod \left((\lambda - 1) \one + c^{\{\f\}}\right)
\end{align*}
 
\paragraph{Base method}
%
\[
  	A^{\{\f,\f\}}=A^{\{\s,\s\}} =
	  	\begin{bmatrix}
 0 & 0 & 0 \\
 c_2 & 0 & 0 \\
 \frac{c_3 \left(3 c_2^2-3 c_2+c_3\right)}{c_2 (3
   c_2-2)} & \frac{c_3 (c_2-c_3)}{c_2 (3 c_2-2)} & 0
	  	\end{bmatrix},
		\quad
c^{{\{\f\}}} =   c^{{\{\s\}}} =	\begin{bmatrix}
 0 \\
 c_2 \\
 c_3
\end{bmatrix},
\]		

\[
b^{{\{\f\}}} =   b^{{\{\s\}}} = \begin{bmatrix}\frac{6 c_2 c_3-3 c_2-3 c_3+2}{6 c_2 c_3} \\
 \frac{2-3 c_3}{6 c_2^2-6 c_2 c_3} \\
 -\frac{2-3 c_2}{6 c_2 c_3-6 c_3^2}
\end{bmatrix}
		\quad
    \widehat{b}^{{\{\f\}}}  =   \widehat{b}^{{\{\s\}}} = \begin{bmatrix}
     \hat{b}_2 \left(\frac{c_2}{c_3}-1\right)-\frac{1}{2 c_3}+1 \\
 \hat{b}_2 \\
 \frac{1-2 \hat{b}_2 c_2}{2 c_3} \\
\end{bmatrix}
\]
%
\paragraph{FS coupling}
%
\[
  A^{\{\f,\s,\lambda\}}  = 
  \begin{cases}
  \frac{1}{M}\,\begin{bmatrix}
	  	\lambda-1 & 0 & 0\\
	  	c_2 + \lambda-1 & 0 & 0\\
	  	c_3 + \lambda-1 & 0 & 0
	  	\end{bmatrix}, & 1 \le \lambda \le L_2, \\[12pt]
  \frac{1}{M}\,\begin{bmatrix}
	  	\alpha^\lambda_{1} &\lambda-1-\alpha^\lambda_{1} & 0 \\
	  	\alpha^\lambda_{2} &c_2 + \lambda-1-\alpha^\lambda_{2} & 0 \\
	  	\alpha^\lambda_{3} &c_3 + \lambda-1-\alpha^\lambda_{3} & 0 
	  	\end{bmatrix}, & L_2+1 \le \lambda \le L_3, \\[12pt]
  \frac{1}{M}\,\begin{bmatrix}
	  	\beta^\lambda_{1,1} &\beta^\lambda_{1,2} &\lambda-1-\beta^\lambda_{1,1} -\beta^\lambda_{1,2}  \\
	  	\beta^\lambda_{2,1} &\beta^\lambda_{2,2} &c_2 + \lambda-1-\beta^\lambda_{2,1} -\beta^\lambda_{2,2}  \\
	  	\beta^\lambda_{3,1} &\beta^\lambda_{3,2} &c_3 + \lambda-1-\beta^\lambda_{3,1} -\beta^\lambda_{3,2} 
	  	\end{bmatrix}, & L_3+1 \le \lambda \le M,
\end{cases}		
\]
%
We will try to choose $\beta^\lambda_{:,1}=0$ if possible, to increase sparsity.
%
\[
b^T\,  A^{\{\f,\s,\lambda\}} \,c = 
  \begin{cases}
  0, & 1 \le \lambda \le L_2, \\[3pt]
(\lambda-1/2-b^T\,\alpha^\lambda_:)\, c_2, & L_2+1 \le \lambda \le L_3, \\[3pt]
(\lambda-1/2-b^T\,\beta^\lambda_{:,1})\, c_3 + (b^T\,\beta^\lambda_{:,2})\, (c_2-c_3), & L_3+1 \le \lambda \le M.
\end{cases}		
\]
%	  	
\begin{align*}
\frac{M}{6}=&\sum_{\lambda=1}^M \tr{b} \mprod A^{\{\f,\s,\lambda\}} \mprod c \\
\frac{M^2}{6}=&\sum_{\lambda=L_2+1}^{L_3} (\lambda-1/2-b^T\,\alpha^\lambda_:)\, c_2 +
\sum_{\lambda=L_3+1}^{M} (\lambda-1/2-b^T\,\beta^\lambda_{:,1})\, c_3 \\
&+ \sum_{\lambda=L_3+1}^{M} (b^T\,\beta^\lambda_{:,2})\, (c_2-c_3) \\
=& \frac{c_2}{2}(L_3^2-L_2^2) +  \frac{c_3}{2}(M^2-L_3^2) - \sum_{\lambda=L_2+1}^{L_3} (b^T\,\alpha^\lambda_:)\, c_2 - \sum_{\lambda=L_3+1}^{M} (b^T\,\beta^\lambda_{:,1})\, c_3 \\
&+ \sum_{\lambda=L_3+1}^{M} (b^T\,\beta^\lambda_{:,2})\, (c_2-c_3)
\end{align*} 
%
One solution is $L_3=M$:
%
\[
\alpha^\lambda_: =\kappa (\lambda-1/2) \one, 
\]
%
for which:
%
\begin{align*}
\frac{M^2}{6}=& \frac{(1-\kappa)c_2}{2}(M^2-L_2^2) 
\quad \Rightarrow \quad 
\kappa = 1-\frac{1}{3c_2(1-L_2^2/M^2)}.
\end{align*} 

Many other solutions are also possible.
%
\paragraph{SF coupling}
%
\[
  A^{\{\s,\f,\lambda\}}  = 
  \begin{cases}
	  	\begin{bmatrix}
	  	0 & 0 & 0\\
	  	\theta^\lambda_1 & \theta^\lambda_2 & \theta^\lambda_3 \\
	  	\mu^\lambda_1 & \mu^\lambda_2 & \mu^\lambda_3
	  	\end{bmatrix}, &  \lambda \le L_2, \\[12pt]
		%
	  	\begin{bmatrix}
	  	0 & 0 & 0\\
	  	0 & 0 & 0\\
	  	\zeta^\lambda_1 & \zeta^\lambda_2 & \zeta^\lambda_3
	  	\end{bmatrix}, & L_2+1 \le \lambda \le L_3, \\[12pt]
		%
	  	\begin{bmatrix}
	  	0 & 0 & 0\\
	  	0 & 0 & 0\\
	  	0 & 0 & 0
	  	\end{bmatrix}, & L_3+1 \le \lambda \le M.
\end{cases}		
\]
%
\begin{align*}
M c_2 &= \sum_{\lambda=1}^{L_2} ( \theta^\lambda_1 + \theta^\lambda_2 + \theta^\lambda_3) \\
M c_3 &= \sum_{\lambda=1}^{L_2} ( \mu^\lambda_1 + \mu^\lambda_2 + \mu^\lambda_3)
+ \sum_{\lambda=L_2+1}^{L_3} ( \zeta^\lambda_1 + \zeta^\lambda_2 + \zeta^\lambda_3)
\end{align*}
%
They can be satisfied by the choice of the first coefficients:
%
\[
\theta^\lambda_1 = \frac{M c_2}{L_2} -\theta^\lambda_2 - \theta^\lambda_3, \quad
\mu^\lambda_1 = -\mu^\lambda_2 - \mu^\lambda_3,\quad
\zeta^\lambda_1 = \frac{M c_3}{L_3-L_2} - \zeta^\lambda_2 - \zeta^\lambda_3
\]

%\[ 
% \tr{b} A^{\{\s,\f,\lambda\}} \mprod \left((\lambda - 1) \one + c\right)
% = 
%\begin{cases}
%b_2 \left( \frac{(\lambda -1) M c_2}{L_2} + \theta^\lambda_{2} c_2 + \theta^\lambda_{3} c_3  \right) + b_3 \left( \mu^\lambda_{2} c_2 + \mu^\lambda_{3} c_3 \right), &  \lambda \le L_2, \\
%%
%b_3 \left( \frac{(\lambda -1) M c_3}{L_3 -L_2} + \zeta^\lambda_{2} c_2 + \zeta^\lambda_{3} c_3 \right), & L_2+1 \le \lambda \le L_3, \\
%0 & L_3+1 \le \lambda \le M.
%\end{cases}
%\]

\begin{align*}
\frac{M^2}{6} &= \sum_{\lambda=1}^M \tr{b^{\{\s\}}} A^{\{\s,\f,\lambda\}} \mprod \left((\lambda - 1) \one + c^{\{\f\}}\right) \\
%
& = b_2  \sum_{\lambda=1}^{L_2}(\lambda-1) (\theta^\lambda_1+ \theta^\lambda_2+ \theta^\lambda_3)
+b_2 \sum_{\lambda=1}^{L_2} (c_2 \theta^\lambda_2 + c_3 \theta^\lambda_3) \\
& \quad +  b_3  \sum_{\lambda=L_2+1}^{L_3} (\lambda-1) (\zeta^\lambda_1 +  \zeta^\lambda_2 + \zeta^\lambda_3) 
	 + b_3  \sum_{\lambda=L_2+1}^{L_3}(c_2 \zeta^\lambda_2 + c_3\zeta^\lambda_3) + b_3  \sum_{\lambda=1}^{L_2}(c_2 \mu^\lambda_2 + c_3\mu^\lambda_3)\\
%
&=  M\frac{b_2 c_2}{L_2}  \sum_{\lambda=1}^{L_2}(\lambda-1) +b_2 \sum_{\lambda=1}^{L_2} (c_2 \theta^\lambda_2 + c_3 \theta^\lambda_3)\\
& \quad + M \frac{b_3 c_3}{L_3-L_2} \sum_{\lambda=L_2+1}^{L_3} (\lambda-1) 
	+ b_3  \sum_{\lambda=L_2+1}^{L_3}(c_2 \zeta^\lambda_2 + c_3\zeta^\lambda_3) + b_3  \sum_{\lambda=1}^{L_2}(c_2 \mu^\lambda_2 + c_3\mu^\lambda_3) \\
% 
&=  \frac{ M b_2 c_2 (L_2-1)}{2} +  b_2  \sum_{\lambda=1}^{L_2}(c_2 \theta^\lambda_2 + c_3\theta^\lambda_3) \\
&\quad + \frac{M b_3 c_3 (L_3+L_2-1)}{2} + b_3  \sum_{\lambda=L_2+1}^{L_3}(c_2 \zeta^\lambda_2 + c_3\zeta^\lambda_3) 
	+ b_3  \sum_{\lambda=1}^{L_2}(c_2 \mu^\lambda_2 + c_3\mu^\lambda_3)
%
\end{align*}
\begin{figure}[ht!]
	\centering
	\begin{subfigure}[b]{0.31\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/Stability/Type-S/EX3-S-M-2.pdf}
		\caption{$M=2$.}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.31\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/Stability/Type-S/EX3-S-M-4.pdf}
		\caption{$M=4$.}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.3\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/Stability/Type-S/EX3-S-M-8.pdf}
		\caption{$M=8$.}
	\end{subfigure}
	\caption{Stability plots for \mgark \method{\explicit}{\explicit}{3}{2}{3}{3}[S] method with $c_2 = \frac{1}{2}$ . }
\end{figure}

For $L_3=M$ we obtain:
\begin{align*}
\frac{M^2}{6} 
=&  M \frac{L_2-1}{4}+\frac{b_3 c_3 M^2}{2}  \\
& + b_2  \sum_{\lambda=1}^{L_2}(c_2 \theta^\lambda_2 + c_3\theta^\lambda_3) +  b_3  \sum_{\lambda=1}^{L_2}(c_2 \mu^\lambda_2 + c_3\mu^\lambda_3)
\end{align*}
%
by parametrize the remaining coupling coefficients as : 
\begin{align*}
	&\zeta _2=k_1 \lambda, \quad  \zeta _3=k_2, \\ 
	&\theta _2=k_3 \lambda, \quad \theta _3=k_4 \lambda, \\
	&\mu _2=k_5 \lambda, \quad \mu _3=k_6 \lambda,
\end{align*}
the slow-fast order condition becomes:
\begin{align*}
\frac{M^2}{6} 
=& M^2 \frac{\left(3 c_2-2\right) \left(c_2 k_1+1\right)}{12 \left(c_2-1\right)}\\
+&M\frac{c_2 \left(-2 k_1+6 k_2+3 L_2-3\right)+3 c_2^2 k_1-4 k_2-3 L_2+3}{12 \left(c_2-1\right)} \\
& -L_2 \frac{3 c_2^3 \left(k_1-k_5\right) \left(L_2+1\right)+c_2^2 \left(-2 k_1 \left(L_2+1\right)+\left(2 k_5-3 k_6\right) \left(L_2+1\right)+6 k_2\right)} {{12 \left(c_2-1\right) c_2}} \\
&\quad + L_2 \frac{c_2 \left(\left(k_3+2 k_6\right) \left(L_2+1\right)-4 k_2\right)+k_4 \left(L_2+1\right)}{12 \left(c_2-1\right) c_2},
\end{align*}
%
with the solution :

\begin{align*}
&k_3 =  -\frac{c_2 \left(c_2 \left(4 L_2-3\right)-3 L_2+3\right)}{\left(c_2-1\right) \left(3 c_2^2+4 c_2+1\right) \left(L_2+1\right)},\\
&k_1 = \frac{1}{2-3 c_2}, \quad k_2= \frac{c_2 \left(4-3 L_2\right)+3 \left(L_2-1\right)}{6 c_2-4},\\
&k_6 = k_5 = k_4 = k_3, 
\end{align*}
The asymptotic behavior of the multirate GARRK matrix is 
\begin{align*}
	\lim_{\substack{L_2 \rightarrow c_2 M\\ M \rightarrow \infty}}\;\Big \vert A_{\textsc{gark}}(i,j) \Big \vert=
	\lim_{\substack{L_2 \rightarrow c_2 M\\ M \rightarrow \infty}}\;\frac{|\zeta_2^\lambda|}{M}   = 2.
\end{align*} 

\subsection{\mgark \method{\explicit}{\implicit}{3}{2}{3}{3}[S]}
\label{subsec:method_EXIM3s}
For an \explicit-\implicit method with stiff accuracy in the slow method we have : 
\[ e_s^T \mprod A^{\{\s,\s}\} = \b^{\{\s\}T}, \quad e_s^T \mprod A^{\{\s,\f\}} = \b^{\{\f\}T}.  \]
This requires that $L_3  = M$ and $\mu_{:} = \zeta_{:} = b^{\{ f \}}$. To keep the method decoupled and have a simple stage computation progression, we couple the first slow stage only with the first fast stage. This requires $L_2 = 1$ . So we have : 
\paragraph{SF coupling}
%
\[
A^{\{\s,\f,\lambda\}}  = 
\begin{cases}
\begin{bmatrix}
M \gamma & 0 & 0\\
\theta^\lambda_1 & \theta^\lambda_2 & 0 \\
b^f_1 &b^f_2 &b^f_3
\end{bmatrix}, &  \lambda = 1, \\[12pt]
%
\begin{bmatrix}
0 & 0 & 0\\
0 & 0 & 0\\
b^f_1 &b^f_2 &b^f_3
\end{bmatrix}, & 2 \le \lambda \le M, \\[12pt]
%
\end{cases}		
\]
%
%
\[
A^{\{\f,\s,\lambda\}}  = 
\begin{cases}
\frac{1}{M}\,\begin{bmatrix}
\lambda-1 & 0 & 0\\
c^{\{\f\}}_2 + \lambda-1 & 0 & 0\\
c^{\{\f\}}_3 + \lambda-1 & 0 & 0
\end{bmatrix}, & 1 \le \lambda \le L_2, \\[12pt]
\frac{1}{M}\,\begin{bmatrix}
\alpha^\lambda_{1} &\lambda-1-\alpha^\lambda_{1} & 0 \\
\alpha^\lambda_{2} &c^{\{\f\}}_2 + \lambda-1-\alpha^\lambda_{2} & 0 \\
\alpha^\lambda_{3} &c^{\{\f\}}_3 + \lambda-1-\alpha^\lambda_{3} & 0 
\end{bmatrix}, & L_2+1 \le \lambda \le M, \\[12pt]
\end{cases}		
\]
%
\[
\theta^\lambda_1 = \frac{M c_2}{L_2} -\theta^\lambda_2 - \theta^\lambda_3, \quad
\]
%
\begin{align*}
\frac{M^2}{6} &= \sum_{\lambda=1}^M \tr{b^{\{\s\}}} A^{\{\s,\f,\lambda\}} \mprod \left((\lambda - 1) \one + c^{\{\f\}}\right) \\
& = \text{b}^s_2 \left(\text{c}^f_3 \left(\text{c}^s_2 M-\theta _1-\theta _2\right)+\text{c}^f_2 \theta _2\right)+\frac{\text{b}^s_3 M^2}{2} \\
& \Rightarrow \theta _2 = \frac{-6 \text{b}^s_2 \text{c}^f_3 \text{c}^s_2 M+6 \text{b}^s_2 \text{c}^f_3 \theta _1-3 \text{b}^s_3 M^2+M^2}{6 \text{b}^s_2 \left(\text{c}^f_2-\text{c}^f_3\right)}
\end{align*}
%
Which scales with $M^2$ unless we can set $b_3^s = 1/3 $ but there are no stiffly accurate SDIRK methods in 3 stages with that coefficient. 
%Solving the fast-to-slow order condition gives :
%\[  \text{c}^f_2=\frac{\gamma -\text{c}^s_2}{3 \gamma -1}  \]
}

==> Include/MGARK_supplementary_material.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Two-partitioned trees of internally consistent methods up to order 4}
\label{sec:ptrees}
%
%
\input{Include/trees_internally_consistent_orders_1-3}
\input{Include/trees_internally_consistent_order_4}
%

==> Include/trees_internally_consistent_order_4.tex <==
%%%%%%%%%%%%%%%%%%%%%%%
\section{Bi-colored trees for internally consistent schemes}
%%%%%%%%%%%%%%%%%%%%%%%
%{\color{blue}
%%%%%%%%%%%%%%%%%%%%%%%
%\section{GARK simplifying assumptions}
%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Simplifying assumptions of type $C(\ell,k)$}
%%%%%%%%%%%%%%%%%%%%%%%
%
%We introduce the following GARK simplifying assumption:
%%
%\begin{eqnarray}
%\label{eqn:simplifying-condition-C}
%C(\ell,k): \qquad \mathbf{A}^{\{\sigma,\mu_1\}} \cdot \dots \cdot \mathbf{A}^{\{\mu_{\ell-1},\mu_\ell\}} \cdot \mathbf{c}^{\{\mu_\ell\} \times k}  &=&  \left( \mathbf{A}^{\{\sigma,\sigma\}} \right)^\ell \cdot \mathbf{c}^{\{\sigma\} \times k}, \quad \\
%\nonumber
%&&\quad \forall~ \sigma,\mu_1,\dots,\mu_\ell.
%\end{eqnarray}
%%
%\begin{table}
%\centering
%\begin{tabular}{||c c c||}
%    \hline\hline
%    \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$$](j){$\sigma$}; [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\mathbf{A}^{\{\sigma,\nu\}}$](k){$\nu$}; [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\mathbf{c}^{\{\nu\}}$](m){$\nu$};  ][.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\mathbf{c}^{\{\nu\}}$](l){$\nu$};  ] ] ]\end{tikzpicture} & 
%    $\longrightarrow$ &
%    \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$$](j){$\sigma$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\mathbf{A}^{\{\sigma,\sigma\}}$](k){$\sigma$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\mathbf{c}^{\{\sigma\}}$](m){$\sigma$};  ][.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\mathbf{c}^{\{\sigma\}}$](l){$\sigma$};  ] ] ]\end{tikzpicture}\\ 
%\hline\hline
%%
%        \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$$](j){$\sigma$}; [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\mathbf{A}^{\{\sigma,\mu_1\}}$](k){$\mu_1$}; [.\node[circle,draw,thick,fill=green!50,opacity=0.5,label=right:$\mathbf{A}^{\{\mu_1,\mu_2\}}$](l){$\mu_2$}; [.\node[circle,draw,thick,fill=green!50,opacity=0.5,label=right:$\mathbf{c}^{\{\mu_2\}}$](m){$\mu_2$};  ] ] ] ]\end{tikzpicture} &
%            $\longrightarrow$ & 
%         \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$$](j){$\sigma$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\mathbf{A}^{\{\sigma,\sigma\}}$](k){$\sigma$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\mathbf{A}^{\{\sigma,\sigma\}}$](l){$\sigma$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\mathbf{c}^{\{\sigma\}}$](m){$\sigma$};  ] ] ] ]\end{tikzpicture} \\ \hline\hline
%%
%\end{tabular}
%\caption{How condition $C(\ell,k)$ \eqref{eqn:simplifying-condition-C} simplifies trees. In the upper two panels $\ell=1$ and $k=2$. In the lower two panels $\ell=2$ and $k=1$. The equation $\mathbf{A}^{\{\sigma,\mu\}} \cdot \mathbf{c}^{\{\mu\} \times k}  =  \mathbf{A}^{\{\sigma,\sigma\}} \cdot \mathbf{c}^{\{\sigma\} \times k}$ means that a subtree with $\ell+1$ levels, consisting of a linear branch that ends with $k$ leaves, gets the color of its root.}
%\end{table}
%
%
%First condition $C(1,1)$ for multirate schemes:
%	\begin{align*}
%	\A^{\{\f,\s\}} \mprod \c^{\{\s\}} &= \A^{\{\f,\f\}} \mprod \c^{\{\f\}} \\
%	\left[ A^{\{\f,\s,\lambda\}} \mprod c^{\{\s\}}\right]_{\lambda=1,\dots,M} 
%	&= \left[ \frac{1}{M^2}\left(\frac{(\lambda-1)^2}{2} \one + (\lambda-1) c^{\{\f\}} + A^{\{\f,\f\}} \mprod  c^{\{\f\}} \right) \right]_{\lambda=1,\dots,M},
%	\end{align*}
%
%Second condition $C(1,1)$ for multirate schemes:
%	\begin{align*}
%	\A^{\{\s,\s\}}\mprod \c^{\{\s\}} &= \A^{\{\s,\f\}}\mprod \c^{\{\f\}} \\
%	A^{\{\s,\s\}}\mprod c^{\{\s\}} &=  \frac{1}{M^2} \sum_{\lambda=1}^M A^{\{\s,\f,\lambda\}} \mprod \left((\lambda - 1) \one + c^{\{\f\}}\right).
%	\end{align*}
%
%%	\begin{align}
%%	%
%%	\c^{\{\f\}} &= \frac{1}{M} \left[ c^{\{\f\}} + \left(\lambda-1\right) \one  \right]_{\lambda=1,\dots,M},\\
%%	%	
%%	\A^{\{\f,\f\}} \mprod \c^{\{\f\}} &= \left[ \frac{1}{M^2}\left(\frac{(\lambda-1)^2}{2} \one + (\lambda-1) c^{\{\f\}} + A^{\{\f,\f\}} \mprod  c^{\{\f\}} \right) \right]_{\lambda=1,\dots,M},\\
%%	%
%%	\A^{\{\s,\f\}}\mprod \c^{\{\f\}}
%%	&= \frac{1}{M^2} \sum_{\lambda=1}^M A^{\{\s,\f,\lambda\}} \mprod \left((\lambda - 1) \one + c^{\{\f\}}\right), \\
%%	%
%%	\A^{\{\f,\f\}} \mprod \A^{\{\f,\s\}} \mprod \c^{\{\s\}} &= \frac{1}{M}\left[ \sum_{k=1}^{\lambda -1} \one \mprod \tr{b^{\{\f\}}} \mprod  A^{\{\f,\s,k\}} \mprod c^{\{\s\}} +  A^{\{\f,\f\}} \mprod A^{\{\f,\s,\lambda\}} \mprod c^{\{\s\}}  \right]_{\lambda=1,\dots,M},
%%	%
%%	\end{align}
%
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Simplifying assumptions of type $D(\ell,k)$}
%%%%%%%%%%%%%%%%%%%%%%%
%%
%\begin{eqnarray}
%\label{eqn:simplifying-condition-D}
%D(\ell,k): && \left(\mathbf{b}^{\{\sigma\}} \times \mathbf{c}^{\{\sigma\} \times k}\right)^T  \cdot \mathbf{A}^{\{\sigma,\mu_1\}}\cdot \dots  \cdot \mathbf{A}^{\{\mu_{\ell-1},\mu_\ell\}} \\
%&=& \left(\mathbf{b}^{\{\mu_\ell\}} \times \mathbf{c}^{\{\mu_\ell\} \times k}\right)^T  \cdot \left( \mathbf{A}^{\{\mu_\ell,\mu_\ell\}} \right)^\ell, \quad \\
%\nonumber
%&& \qquad\forall~ \sigma,\mu_1,\dots,\mu_\ell.
%\end{eqnarray}
%%
%The way condition $D(\ell,k)$ simplifies trees is illustrated in Table \ref{tab:simplifying-condition-D}.
%%
%\begin{table}[hp]
%\centering
%\begin{tabular}{||c c c ||}
%    \hline\hline
%    \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\mathbf{b}^{\{\sigma\}}\,^T$](j){$\sigma$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\mathbf{A}^{\{\sigma,\nu\}}$](l){$\nu$};  ][.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\mathbf{c}^{\{\sigma\}}$](k){$\sigma$};  ] ]\end{tikzpicture} 
%    & $\longrightarrow$ & 
%    \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\mathbf{b}^{\{\nu\}}\,^T$](j){$\nu$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\mathbf{A}^{\{\nu,\nu\}}$](l){$\nu$};  ][.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\mathbf{c}^{\{\nu\}}$](k){$\nu$};  ] ]\end{tikzpicture} \\ 
%    \hline\hline
%\end{tabular}
%\caption{How condition $D(\ell,k)$ simplifies trees. Here $\ell=k=1$. A tree has a root with $k+1$ children, out of which $k$ are leaves. The $k+1$-st is a subtree that starts with $\ell$ nodes in a linear pattern. The root takes the color of the $\ell$-th child of its $k+1$-st child.}
%\label{tab:simplifying-condition-D}
%\end{table}
%
%First condition $D(1,0)$ for multirate schemes:
%%
%\begin{align*}
%	\b^{\{\f\}}\,^T \mprod  \A^{\{\f,\s\}}   &= \b^{\{\s\}}\,^T \mprod \A^{\{\s,\s\}}  \\
%\frac{1}{M}\,\sum_{\lambda=1}^M b^{\{\f\}}\,^T A^{\{\f,\s,\lambda\}}&= b^{\{\s\}}\,^T \mprod A^{\{\s,\s\}}
%\end{align*}
%%
%Second condition $D(1,0)$ for multirate schemes:
%%
%\begin{align*}
%	\b^{\{\s\}}\,^T \mprod \A^{\{\s,\f\}}  &= \b^{\{\f\}}\,^T \mprod \A^{\{\f,\f\}}  \\
%	\left[ b^{\{\s\}}\,^T \mprod A^{\{\s,\f,\lambda\}} \right]_{\lambda} &= \left[ \frac{1}{M}\,b^{\{\f\}}\,^T \mprod A^{\{\f,\f\}} + \frac{M-\lambda}{M}\,b^{\{\f\}}\,^T \right]_{\lambda}
%\end{align*}
%
%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Consequences of simplifying assumptions}
%%%%%%%%%%%%%%%%%%%%%%%
%
%\begin{lemma}
%Internal consistency is the property $C(1,0)$ \eqref{eqn:simplifying-condition-C}.
%\end{lemma}
%
%\begin{lemma}
%For internally consistent MR-GARK methods satisfying the simplifying conditions \eqref{eqn:simplifying-condition-C} with $C(1,1)$:
%%
%\begin{itemize}
%\item There are no coupling conditions of order 2.
%\item There are no coupling conditions of order 3. This property is enjoyed equally by the main and by any embedded methods.
%\item The order 4 conditions simplify considerably, as follows:
%\begin{itemize}
%\item The two trees in table \ref{tab:N2t41_intconsist} remain the same
%\item Only $t_{4,2}^{\langle 2,1 \rangle}$ and $t_{4,2}^{\langle 2,16 \rangle}$ remain from the trees of table \ref{tab:N2t42_intconsist}
%\item The four trees in table \ref{tab:N2t43_intconsist} remain the same
%\item Only $t_{4,4}^{\langle 2,1 \rangle}$, $t_{4,4}^{\langle 2,8 \rangle}$, $t_{4,4}^{\langle 2,9 \rangle}$, $t_{4,4}^{\langle 2,16 \rangle}$ remain from the trees of table \ref{tab:N2t44_intconsist}.
%\end{itemize}
%\item Among the 11 trees for order 4 only $t_{4,3}^{\langle 2,6 \rangle}$, $t_{4,3}^{\langle 2,7 \rangle}$, $t_{4,4}^{\langle 2,8 \rangle}$, and $t_{4,4}^{\langle 2,9 \rangle}$ represent coupling conditions.
%\end{itemize}
%\end{lemma}
%
%\begin{lemma}
%For internally consistent MR-GARK methods satisfying the simplifying conditions $D(1,0)$ \eqref{eqn:simplifying-condition-D}:
%%
%\begin{itemize}
%\item There are no coupling conditions of order 2.
%\item There are no coupling conditions of order 3. This property is enjoyed equally by the main and by any embedded methods.
%\item the order 4 conditions simplify considerably, as follows:
%\begin{itemize}
%\item The two trees in table \ref{tab:N2t41_intconsist} remain the same
%\item Only $t_{4,2}^{\langle 2,1 \rangle}$ and $t_{4,2}^{\langle 2,16 \rangle}$ remain from the trees of table \ref{tab:N2t42_intconsist}
%\item The four trees in table \ref{tab:N2t43_intconsist} remain the same
%\item Only $t_{4,4}^{\langle 2,1 \rangle}$, $t_{4,4}^{\langle 2,8 \rangle}$, $t_{4,4}^{\langle 2,9 \rangle}$, $t_{4,4}^{\langle 2,16 \rangle}$ remain from the trees of table \ref{tab:N2t44_intconsist}.
%\end{itemize}
%\item Among the 11 trees for order 4 only $t_{4,3}^{\langle 2,6 \rangle}$, $t_{4,3}^{\langle 2,7 \rangle}$, $t_{4,4}^{\langle 2,8 \rangle}$, and $t_{4,4}^{\langle 2,9 \rangle}$ represent coupling conditions.
%\end{itemize}
%\end{lemma}
%
%\begin{lemma}
%For MR-GARK methods satisfying the simplifying conditions $C(1,0) \&C(1,1)\&D(1,0)$, or $C(1,0) \&C(1,1)\&C(2,1)$:
%%
%\begin{itemize}
%\item There are no coupling conditions of order 2.
%\item There are no coupling conditions of order 3. 
%\item There are no coupling conditions of order 4.
%\end{itemize}
%\end{lemma}
%}


\bgroup
\def\arraystretch{1.5}

\begin{table}[hp]
\centering
\begin{tabular}{||c ||c ||}
\hline\hline
    \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\tr{\b^{\{\s\}}}$](j){$\s$}; [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\c^{\{\s\}}$](m){$\s$};  ][.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\c^{\{\s\}}$](l){$\s$};  ][.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\c^{\{\s\}}$](k){$\s$};  ] ]\end{tikzpicture} & 
    \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\tr{\b^{\{\f\}}}$](j){$\f$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\c^{\{\f\}}$](m){$\f$};  ][.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\c^{\{\f\}}$](l){$\f$};  ][.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\c^{\{\f\}}$](k){$\f$};  ] ]\end{tikzpicture} \\ \hline
$t_{4,1}^{\langle 2,1 \rangle}$ &  $t_{4,1}^{\langle 2,8 \rangle}$ \\ \hline
    $\tr{\b^{\{\s\}}} \mprod \c^{\{\s\} \times 3} = \frac{1}{4}$ & 
    $\tr{\b^{\{\f\}}} \mprod \c^{\{\f\} \times 3} = \frac{1}{4}$ \\ \hline\hline
\end{tabular}
\caption{Internally consistent $N2T$-trees corresponding to $t_{4,1}$. In total there are 8 $N2T$-trees generated by $t_{4,1}$.}
\label{tab:N2t41_intconsist}
\end{table}

\begin{table}[hp] \centering
\begin{tabular}{||c ||c ||}
\hline\hline
    \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\tr{\b^{\{\s\}}}$](j){$\s$}; [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\A^{\{\s,\s\}}$](l){$\s$}; [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\c^{\{\s\}}$](m){$\s$};  ] ][.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\c^{\{\s\}}$](k){$\s$};  ] ]\end{tikzpicture} & 
  \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\tr{\b^{\{\s\}}}$](j){$\s$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\A^{\{\s,\f\}}$](l){$\f$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\c^{\{\f\}}$](m){$\f$};  ] ][.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\c^{\{\s\}}$](k){$\s$};  ] ]\end{tikzpicture}  \\ \hline
$t_{4,2}^{\langle 2,1 \rangle}$ &  $t_{4,2}^{\langle 2,4 \rangle}$ \\ \hline
    $\tr{\b^{\{\s\}}} \mprod\left( \c^{\{\s\}} \sprod \A^{\{\s,\s\}} \mprod \c^{\{\s\}}\right)= \frac{1}{8}$ & 
    $\tr{\b^{\{\s\}}} \mprod \left( \c^{\{\s\}}\sprod \A^{\{\s,\f\}} \mprod  \c^{\{\f\}} \right)= \frac{1}{8}$ \\ \hline\hline
%
    \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\tr{\b^{\{\f\}}}$](j){$\f$}; [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\A^{\{\f,\s\}}$](l){$\s$}; [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\c^{\{\s\}}$](m){$\s$};  ] ][.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\c^{\{\f\}}$](k){$\f$};  ] ]\end{tikzpicture} & 
   \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\tr{\b^{\{\f\}}}$](j){$\f$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\A^{\{\f,\f\}}$](l){$\f$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\c^{\{\f\}}$](m){$\f$};  ] ][.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\c^{\{\f\}}$](k){$\f$};  ] ]\end{tikzpicture} \\ \hline
$t_{4,2}^{\langle 2,13 \rangle}$ &  $t_{4,2}^{\langle 2,16 \rangle}$ \\ \hline
    $\tr{\b^{\{\f\}}} \mprod \left(\c^{\{\f\}} \sprod \A^{\{\f,\s\}} \c^{\{\s\}} \right)= \frac{1}{8}$ &
    $\tr{\b^{\{\f\}}} \mprod \left( \c^{\{\f\}} \sprod \A^{\{\f,\f\}} \mprod \c^{\{\f\}} \right)= \frac{1}{8}$ \\ \hline\hline
\end{tabular}
\caption{Internally consistent $N2T$-trees corresponding to $t_{4,2}$. In total there are 16 $N2T$-trees generated by $t_{4,2}$.}
\label{tab:N2t42_intconsist}
\end{table}


\begin{table}[hp] \centering
\begin{tabular}{||c ||c ||}
    \hline\hline
    \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\tr{\b^{\{\s\}}}$](j){$\s$}; [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$ \A^{\{\s,\s\}}$](k){$\s$}; [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\c^{\{\s\}}$](m){$\s$};  ][.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\c^{\{\s\}}$](l){$\s$};  ] ] ]\end{tikzpicture} & 
    \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\tr{\b^{\{\s\}}}$](j){$\s$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\A^{\{\s,\f\}}$](k){$\f$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\c^{\{\f\}}$](m){$\f$};  ][.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\c^{\{\f\}}$](l){$\f$};  ] ] ]\end{tikzpicture}\\ \hline
$t_{4,3}^{\langle 2,1 \rangle}$ &  $t_{4,3}^{\langle 2,6 \rangle}$ \\ \hline
    $\tr{\b^{\{\s\}}} \mprod \A^{\{\s,\s\}} \mprod \c^{\{\s\}\times 2} = \frac{1}{12}$ & 
    $\tr{\b^{\{\s\}}} \mprod \A^{\{\s,\f\}} \mprod \c^{\{\f\}\times 2} = \frac{1}{12}$ \\ \hline\hline
    %
    \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\tr{\b^{\{\f\}}}$](j){$\f$}; [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\A^{\{\f,\s\}}$](k){$\s$}; [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\c^{\{\s\}}$](m){$\s$};  ][.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\c^{\{\s\}}$](l){$\s$};  ] ] ]\end{tikzpicture} & 
    \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\tr{\b^{\{\f\}}}$](j){$\f$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\A^{\{\f,\f\}}$](k){$\f$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\c^{\{\f\}}$](m){$\f$};  ][.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\c^{\{\f\}}$](l){$\f$};  ] ] ]\end{tikzpicture}\\ \hline
 $t_{4,3}^{\langle 2,7 \rangle}$ &  $t_{4,3}^{\langle 2,12 \rangle}$\\ \hline
    $\tr{\b^{\{\f\}}} \mprod \A^{\{\f,\s\}} \mprod \c^{\{\s\}\times 2} = \frac{1}{12}$ & 
    $\tr{\b^{\{\f\}}} \mprod \A^{\{\f,\f\}} \mprod \c^{\{\f\}\times 2}  = \frac{1}{12}$ \\
\hline\hline
\end{tabular}
\caption{Internally consistent $N2T$-trees corresponding to $t_{4,3}$. In total there are 12 $N2T$-trees generated by $t_{4,3}$.}
\label{tab:N2t43_intconsist}
\end{table}



\begin{table}[hp] \centering
\begin{tabular}{||c ||c ||}
    \hline\hline
    \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\tr{\b^{\{\s\}}}$](j){$\s$}; [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\A^{\{\s,\s\}}$](k){$\s$}; [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\A^{\{\s,\s\}}$](l){$\s$}; [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\c^{\{\s\}}$](m){$\s$};  ] ] ] ]\end{tikzpicture} & 
     \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\tr{\b^{\{\s\}}}$](j){$\s$}; [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\A^{\{\s,\s\}}$](k){$\s$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\A^{\{\s,\f\}}$](l){$\f$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\c^{\{\f\}}$](m){$\f$};  ] ] ] ]\end{tikzpicture} \\ \hline
$t_{4,4}^{\langle 2,1 \rangle}$ &   $t_{4,4}^{\langle 2,4 \rangle}$ \\ \hline
    $\tr{\b^{\{\s\}}} \mprod \A^{\{\s,\s\}}\mprod \A^{\{\s,\s\}} \mprod \c^{\{\s\}} = \frac{1}{24}$ 
    & $\tr{\b^{\{\s\}}} \mprod \A^{\{\s,\s\}} \mprod \A^{\{\s,\f\}} \mprod \c^{\{\f\}} = \frac{1}{24}$ \\ \hline\hline
    %
    \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\tr{\b^{\{\s\}}}$](j){$\s$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\A^{\{\s,\f\}}$](k){$\f$}; [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\A^{\{\f,\s\}}$](l){$\s$}; [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\c^{\{\s\}}$](m){$\s$};  ] ] ] ]\end{tikzpicture} & 
    \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\tr{\b^{\{\s\}}}$](j){$\s$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\A^{\{\s,\f\}}$](k){$\f$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\A^{\{\f,\f\}}$](l){$\f$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\c^{\{\f\}}$](m){$\f$};  ] ] ] ]\end{tikzpicture} \\ \hline    
$t_{4,4}^{\langle 2,5 \rangle}$ &   $t_{4,4}^{\langle 2,8 \rangle}$ \\ \hline
    $\tr{\b^{\{\s\}}} \mprod \A^{\{\s,\f\}} \mprod \A^{\{\f,\s\}} \mprod  \c^{\{\s\}} = \frac{1}{24}$ & 
    $\tr{\b^{\{\s\}}} \mprod \A^{\{\s,\f\}} \mprod \A^{\{\f,\f\}} \mprod  \c^{\{\f\}} = \frac{1}{24}$ \\     \hline\hline
%
        \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\tr{\b^{\{\f\}}}$](j){$\f$}; [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\A^{\{\f,\s\}}$](k){$\s$}; [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\A^{\{\s,\s\}}$](l){$\s$}; [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\c^{\{\s\}}$](m){$\s$};  ] ] ] ]\end{tikzpicture} & 
         \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\tr{\b^{\{\f\}}}$](j){$\f$}; [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\A^{\{\f,\s\}}$](k){$\s$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\A^{\{\s,\f\}}$](l){$\f$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\c^{\{\f\}}$](m){$\f$};  ] ] ] ]\end{tikzpicture} \\ \hline
$t_{4,4}^{\langle 2,9 \rangle}$ &  $t_{4,4}^{\langle 2,12 \rangle}$ \\ \hline
    $\tr{\b^{\{\f\}}} \mprod \A^{\{\f,\s\}} \mprod \A^{\{\s,\s\}} \mprod  \c^{\{\s\}} = \frac{1}{24}$ & 
    $\tr{\b^{\{\f\}}} \mprod \A^{\{\f,\s\}} \mprod \A^{\{\s,\f\}} \mprod  \c^{\{\f\}} = \frac{1}{24}$ \\ 
\hline\hline
%
    \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\tr{\b^{\{\f\}}}$](j){$\f$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\A^{\{\f,\f\}}$](k){$\f$}; [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\A^{\{\f,\s\}}$](l){$\s$}; [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\c^{\{\s\}}$](m){$\s$};  ] ] ] ]\end{tikzpicture} & 
   \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\tr{\b^{\{\f\}}}$](j){$\f$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\A^{\{\f,\f\}}$](k){$\f$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\A^{\{\f,\f\}}$](l){$\f$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\c^{\{\f\}}$](m){$\f$};  ] ] ] ]\end{tikzpicture} \\ \hline
$t_{4,4}^{\langle 2,13 \rangle}$ &  $t_{4,4}^{\langle 2,16 \rangle}$ \\ \hline
    $\tr{\b^{\{\f\}}} \mprod \A^{\{\f,\f\}} \mprod \A^{\{\f,\s\}} \mprod  \c^{\{\s\}} = \frac{1}{24}$ & 
    $\tr{\b^{\{\f\}}} \mprod \A^{\{\f,\f\}} \mprod \A^{\{\f,\f\}} \mprod  \c^{\{\f\}} = \frac{1}{24}$\\     \hline\hline
    \end{tabular}
\caption{Internally consistent $N2T$-trees corresponding to $t_{4,4}$. In total there are 16 $N2T$-trees generated by $t_{4,4}$.}
\label{tab:N2t44_intconsist}
\end{table}
\egroup

==> Include/trees_internally_consistent_orders_1-3.tex <==
\bgroup
\def\arraystretch{1.5}

\begin{table}[hp]
\centering
\begin{tabular}{||c ||c ||}
    \hline\hline
    \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\tr{\b^{\{\s\}}}$](j){$\s$};  ]\end{tikzpicture} & \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\tr{\b^{\{\f\}}}$](j){$\f$};  ]\end{tikzpicture}\\ \hline
%    $f^{\{\s\}}$ & $f^{\{\f\}}$\\ \hline
$t_{1}^{\langle 2,1 \rangle}$ & $t_{1}^{\langle 2,2 \rangle}$ \\ \hline
    $\tr{\b^{\{\s\}}}\mprod \one = 1$ & $\tr{\b^{\{\f\}}}\mprod \one = 1$ \\ \hline \hline
 %   
    \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\tr{\b^{\{\s\}}}$](j){$\s$}; [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\c^{\{\s\}}$](k){$\s$};  ] ]\end{tikzpicture} & 
    \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\tr{\b^{\{\f\}}}$](j){$\f$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\c^{\{\f\}}$](k){$\f$};  ] ]\end{tikzpicture}\\ \hline
$t_{2}^{\langle 2,1 \rangle}$ & $t_{2}^{\langle 2,4 \rangle}$ \\ \hline
    $\tr{\b^{\{\s\}}} \mprod \c^{\{\s\}} = \frac{1}{2}$ & 
    $\tr{\b^{\{\f\}}} \mprod\c^{\{\f\}} = \frac{1}{2}$ \\ \hline \hline
\end{tabular}
\caption{N2T-trees up to order 2 for internally consistent methods.}
\label{tab:N2T-trees_1-2_intconsistent}
\end{table}

\begin{table}[hp]
\centering\begin{tabular}{||c ||c ||}
    \hline\hline
    \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\tr{\b^{\{\s\}}}$](j){$\s$}; [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\c^{\{\s\}}$](l){$\s$};  ][.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\c^{\{\s\}}$](k){$\s$};  ] ]\end{tikzpicture} & \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\tr{\b^{\{\f\}}}$](j){$\f$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\c^{\{\f\}}$](l){$\f$};  ][.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\c^{\{\f\}}$](k){$\f$};  ] ]\end{tikzpicture} \\ 
    \hline
$t_{3,1}^{\langle 2,1 \rangle}$ &  $t_{3,1}^{\langle 2,6 \rangle}$ \\ \hline
    $\tr{\b^{\{\s\}}} \mprod \c^{\{\s\} \times 2}= \frac{1}{3}$ & 
    $\tr{\b^{\{\f\}}} \mprod \c^{\{\f\} \times 2}= \frac{1}{3}$ \\ \hline \hline
%
    \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\tr{\b^{\{\s\}}}$](j){$\s$}; [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$ \A^{\{\s,\s\}}$](k){$\s$}; [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$ \c^{\{\s\}}$](l){$\s$};  ] ] ]\end{tikzpicture} & 
   \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$\tr{\b^{\{\s\}}}$](j){$\s$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$ \A^{\{\s,\f\}}$](k){$\f$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$ \c^{\{\f\}}$](l){$\f$};  ] ] ]\end{tikzpicture} \\ \hline
$t_{3,2}^{\langle 2,1 \rangle}$ &  $t_{3,2}^{\langle 2,4 \rangle}$ \\ \hline
    $\tr{\b^{\{\s\}}} \mprod \A^{\{\s,\s\}} \mprod \c^{\{\s\}}= \frac{1}{6}$ &  
    $\tr{\b^{\{\s\}}} \mprod \A^{\{\s,\f\}} \mprod \c^{\{\f\}}= \frac{1}{6}$ \\ \hline \hline
    %
    \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\tr{\b^{\{\f\}}}$](j){$\f$}; [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$ \A^{\{\f,\s\}}$](k){$\s$}; [.\node[circle,draw,thick,fill=blue!50,opacity=0.5,label=right:$ \c^{\{\s\}}$](l){$\s$};  ] ] ]\end{tikzpicture} & 
 \begin{tikzpicture}[grow=up]\Tree [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\tr{\b^{\{\f\}}}$](j){$\f$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$\A^{\{\f,\f\}}$](k){$\f$}; [.\node[circle,draw,thick,fill=red!50,opacity=0.5,label=right:$ \c^{\{\f\}}$](l){$\f$};  ] ] ]\end{tikzpicture}   \\ \hline
$t_{3,2}^{\langle 2,5 \rangle}$ &  $t_{3,2}^{\langle 2,8 \rangle}$ \\ \hline
    $\tr{\b^{\{\f\}}} \mprod \A^{\{\f,\s\}} \mprod \c^{\{\s\}} = \frac{1}{6}$ &  
    $\tr{\b^{\{\f\}}} \mprod \A^{\{\f,\f\}} \mprod \c^{\{\f\}} = \frac{1}{6}$ \\ \hline \hline
    \end{tabular}
\caption{N2T-trees of order 3 for internally consistent methods.
}
\label{tab:N2T-trees_3_intconsistent}
\end{table}
\egroup
